Understanding and Finding JIT Compiler Performance Bugs

Just-in-time (JIT) compilers are key components for many popular programming languages with managed runtimes (e.g., Java and JavaScript). JIT compilers perform optimizations and generate native code at runtime based on dynamic profiling data, to improve the execution performance of the running application. Like other software systems, JIT compilers might have software bugs, and prior work has developed a number of automated techniques for detecting functional bugs (i.e., generated native code does not semantically match that of the original code). However, no prior work has targeted JIT compiler performance bugs, which can cause significant performance degradation while an application is running. These performance bugs are challenging to detect due to the complexity and dynamic nature of JIT compilers. In this paper, we present the first work on demystifying JIT performance bugs. First, we perform an empirical study across four popular JIT compilers for Java and JavaScript. Our manual analysis of 191 bug reports uncovers common triggers of performance bugs, patterns in which these bugs manifest, and their root causes. Second, informed by these insights, we propose layered differential performance testing, a lightweight technique to automatically detect JIT compiler performance bugs, and implement it in a tool called Jittery. We incorporate practical optimizations into Jittery such as test prioritization, which reduces testing time by 92.40% without compromising bug-detection capability, and automatic filtering of false-positives and duplicates, which substantially reduces manual inspection effort. Using Jittery, we discovered 12 previously unknown performance bugs in the Oracle HotSpot and Graal JIT compilers, with 11 confirmed and 6 fixed by developers.

==> code/fig-eval-bug1.tex <==
\begin{figure}[t]
    \centering
    \lstinputlisting[language=java-pretty]{code/bug1.java}
    % \vspace{-10pt}
    \caption{\JDKBug{JDK-8346989}}
    \label{fig:eval-bug1}
\end{figure}


==> code/fig-eval-bug2.tex <==
\begin{figure}[t]
    \centering
    \lstinputlisting[language=java-pretty]{code/bug2.java}
    % \vspace{-10pt}
    \caption{\JDKBug{JDK-8349452}}
    \label{fig:eval-bug2}
\end{figure}


==> code/fig-example.tex <==
\begin{figure}[t]
    \lstinputlisting[language=java-pretty]{code/math23-reduced.java}
    \vspace{-10pt}
    \caption{Example of missed optimization in Oracle JDK}
    \label{fig:example}
\end{figure}


==> tables/eval/table-tdt-topk500_100_50.tex <==
%%Auto-generated from table.py
\begin{table*}[t]
\centering
\scriptsize
\caption{Results of Tiered Differential Testing with \Lejit~(Top-K=500, 100, 50). \label{table-eval:tdt-topk500_100_50}}
\begin{tabular}{lcccccccccccc}
\toprule
\multirow2{*}{\centering \textbf{Project}} & \multicolumn2{c}{\textbf{Input}} & \multirow2{*}{\centering \textbf{Pair}} & \multicolumn5{c}{\textbf{Tiered Filtering}} & \multirow2{*}{\textbf{\shortstack{Duplicate\\Filtering}}} & \multirow2{*}{\textbf{\#FP}} & \multirow2{*}{\textbf{\#Bug}} & \multirow2{*}{\textbf{Time [min]}} \\
\cmidrule(lr){2-3} \cmidrule(lr){5-9}
 & \#Template & \#Gen & & $TH_0$ & $TH_1$ & $TH_2$ & $TH_3$ & $TH_4$ & & & & \\
\midrule
\multirow{6}{*}{codec} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-codec-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-codec-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-codec-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-codec-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-codec-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-codec-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-codec-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-codec-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-codec-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-codec-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-codec-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-codec-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-codec-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-codec-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-codec-rp1-tp} & \\
\midrule
\multirow{6}{*}{compress} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-compress-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-compress-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-compress-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-compress-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-compress-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-compress-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-compress-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-compress-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-compress-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-compress-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-compress-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-compress-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-compress-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-compress-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-compress-rp1-tp} & \\
\midrule
\multirow{6}{*}{math} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-math-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-math-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-math-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-math-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-math-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-math-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-math-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-math-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-math-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-math-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-math-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-math-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-math-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-math-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-math-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-math-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-math-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-math-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-math-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-math-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-math-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-math-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-math-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-math-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-math-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-math-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-math-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-math-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-math-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-math-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-math-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-math-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-math-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-math-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-math-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-math-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-math-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-math-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-math-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-math-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-math-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-math-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-math-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-math-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-math-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-math-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-math-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-math-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-math-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-math-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-math-rp1-tp} & \\
\midrule
\multirow{6}{*}{statistics} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-statistics-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-statistics-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-statistics-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-statistics-rp1-tp} & \\
\midrule
\multirow{6}{*}{text} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-text-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-text-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-text-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-text-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-text-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-text-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-text-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-text-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-text-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-text-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-text-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-text-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-text-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-text-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-text-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-text-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-text-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-text-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-text-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-text-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-text-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-text-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-text-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-text-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-text-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-text-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-text-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-text-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-text-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-text-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-text-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-text-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-text-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-text-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-text-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-text-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-text-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-text-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-text-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-text-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-text-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-text-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-text-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-text-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-text-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-text-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-text-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-text-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-text-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-text-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-text-rp1-tp} & \\
\midrule
\multirow{6}{*}{vectorz} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-vectorz-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-vectorz-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-vectorz-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-vectorz-rp1-tp} & \\
\midrule
\multirow{6}{*}{zxing} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-zxing-tmpl}} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-zxing-gen}} & LP0 & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-lp0-tp} & \multirow{6}{*}{\UseMacro{table-tdt-topk500_100_50-zxing-time}} \\
 &  &  & LP1 & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-lp1-tp} & \\
 &  &  & LP2 & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-lp2-tp} & \\
 &  &  & LP3 & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-lp3-tp} & \\
 &  &  & RP0 & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-rp0-tp} & \\
 &  &  & RP1 & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-th0} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-th1} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-th2} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-th3} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-th4} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-fp} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-dup} & \UseMacro{table-tdt-topk500_100_50-zxing-rp1-tp} & \\
\bottomrule
\end{tabular}
\end{table*}

